Realizations of Indecomposable Persistence Modules of Arbitrarily Large Dimension

While persistent homology has taken strides towards becoming a wide-spread tool for data analysis, multidimensional persistence has proven more difficult to apply. One reason is the serious drawback of no longer having a concise and complete descriptor analogous to the persistence diagrams of the former. We propose a simple algebraic construction to illustrate the existence of infinite families of indecomposable persistence modules over regular grids of sufficient size. On top of providing a constructive proof of representation infinite type, we also provide realizations by topological spaces and Vietoris-Rips filtrations, showing that they can actually appear in real data and are not the product of degeneracies.

==> drawing_macros.tex <==
\newcommand\definesandalpts{
  \coordinate (Ia) at (0,1,0);
  \coordinate (Ib) at (0,1,1);
  \coordinate (Sa) at (0,0,0);
  \coordinate (Sb) at (0,0,1);
  \coordinate (Sc) at (1,0,1);
  \coordinate (Sd) at (1,0,0);
  \coordinate (Id) at (1,1,0);
  \coordinate (Ic) at (1,1,1);

  % shrunk
  \coordinate (IaSh) at (0,1,0.2);
  \coordinate (IbSh) at (0,1,0.8);
  \coordinate (SaSh) at (0,0,0.2);
  \coordinate (SbSh) at (0,0,0.8);
  \coordinate (ScSh) at (0.8,0,0.8);
  \coordinate (SdSh) at (0.8,0,0.2);
  \coordinate (IdSh) at (0.8,0.8,0);

  \coordinate (IaEx) at (0,1,-0.2);
  \coordinate (IbEx) at (0,1,1.2);
  \coordinate (SaEx) at (0,0,-0.2);
  \coordinate (SbEx) at (0,0,1.2);
  \coordinate (ScEx) at (1.2,0,1.2);
  \coordinate (SdEx) at (1.2,0,-0.2);
  \coordinate (IdEx) at (1.2,1.2,0);
}

\colorlet{UpperRowColor1}{violet!70!red}
\colorlet{UpperRowColor2}{green!70!black}

\colorlet{LowerRowColor2}{red!70!orange}
\colorlet{LowerRowColor1}{blue!70!violet}

\newcommand{\shiftpt}[2]{
  ($ #1 + (0,2*#2,0) $)
}

\newcommand{\shiftptno}[3]{
  ($ #1 + (2*#3,2*#2,0) $)
 }
  
% Space drawing
\newcommand{\drawuphk}[2]{
  \draw[rounded corners=2pt, #1] \shiftpt{(Sa)}{#2} -- \shiftpt{(Ia)}{#2} -- \shiftpt{(Ib)}{#2} -- \shiftpt{(Sb)}{#2};
}
\newcommand{\drawdwhk}[2]{
  \draw[rounded corners=2pt, #1] \shiftpt{(Sa)}{#2} -- \shiftpt{(Ia)}{#2 - 2}-- \shiftpt{(Ib)}{#2-2} -- \shiftpt{(Sb)}{#2};
}

\newcommand{\drawstrp}[2]{
  \draw[rounded corners=2pt, #1] \shiftpt{(Sb)}{#2} -- \shiftpt{(Sc)}{#2} -- \shiftpt{(Sd)}{#2} -- \shiftpt{(Sa)}{#2};
}

% cycle drawing: shrunk
\newcommand{\shrunkuphk}[2]{
  \draw[rounded corners=2pt, #1] \shiftpt{(SaSh)}{#2} -- \shiftpt{(IaSh)}{#2} -- \shiftpt{(IbSh)}{#2} -- \shiftpt{(SbSh)}{#2};
}
\newcommand{\shrunkdwhk}[2]{
  \draw[rounded corners=2pt, #1] \shiftpt{(SaSh)}{#2} -- \shiftpt{(IaSh)}{#2 - 2}-- \shiftpt{(IbSh)}{#2-2} -- \shiftpt{(SbSh)}{#2};
}

\newcommand{\shrunkstrp}[2]{
  \draw[rounded corners=2pt, #1] \shiftpt{(SbSh)}{#2} -- \shiftpt{(ScSh)}{#2} -- \shiftpt{(SdSh)}{#2} -- \shiftpt{(SaSh)}{#2};
}

% cycle drawing: expand
\newcommand{\expanduphk}[3]{
  \draw[rounded corners=2pt, #1] \shiftpt{(SaEx)}{#3} -- \shiftpt{(IaEx)}{#2} -- \shiftpt{(IbEx)}{#2} -- \shiftpt{(SbEx)}{#3};
}
\newcommand{\expanddwhk}[3]{
  \draw[rounded corners=2pt, #1] \shiftpt{(SaEx)}{#3} -- \shiftpt{(IaEx)}{#2 - 2}-- \shiftpt{(IbEx)}{#2-2} -- \shiftpt{(SbEx)}{#3};
}

\newcommand{\expanduplegs}[3]{
  \draw[#1] \shiftpt{(SaEx)}{#3} -- \shiftpt{(IaEx)}{#2};
  \draw[#1] \shiftpt{(IbEx)}{#2} -- \shiftpt{(SbEx)}{#3};
}
\newcommand{\expanddwlegs}[3]{
  \draw[#1] \shiftpt{(SaEx)}{#3} -- \shiftpt{(IaEx)}{#2 - 2};
  \draw[#1] \shiftpt{(IbEx)}{#2-2} -- \shiftpt{(SbEx)}{#3};
}

\newcommand{\expandstrp}[2]{
  \draw[rounded corners=2pt, #1] \shiftpt{(SbEx)}{#2} -- \shiftpt{(ScEx)}{#2} -- \shiftpt{(SdEx)}{#2} -- \shiftpt{(SaEx)}{#2};
}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "jitsugen_journal"
%%% End:

